High Dimensional Robust $M$-Estimation: Arbitrary Corruption and Heavy Tails

We consider the problem of sparsity-constrained $M$-estimation when both explanatory and response variables have heavy tails (bounded 4-th moments), or a fraction of arbitrary corruptions. We focus on the $k$-sparse, high-dimensional regime where the number of variables $d$ and the sample size $n$ are related through $n \sim k \log d$. We define a natural condition we call the Robust Descent Condition (RDC), and show that if a gradient estimator satisfies the RDC, then Robust Hard Thresholding (IHT using this gradient estimator), is guaranteed to obtain good statistical rates. The contribution of this paper is in showing that this RDC is a flexible enough concept to recover known results, and obtain new robustness results. Specifically, new results include: (a) For $k$-sparse high-dimensional linear- and logistic-regression with heavy tail (bounded 4-th moment) explanatory and response variables, a linear-time-computable median-of-means gradient estimator satisfies the RDC, and hence Robust Hard Thresholding is minimax optimal; (b) When instead of heavy tails we have $O(1/\sqrt{k}\log(nd))$-fraction of arbitrary corruptions in explanatory and response variables, a near linear-time computable trimmed gradient estimator satisfies the RDC, and hence Robust Hard Thresholding is minimax optimal. We demonstrate the effectiveness of our approach in sparse linear, logistic regression, and sparse precision matrix estimation on synthetic and real-world US equities data.

==> Discussion.tex <==

\section{Discussion}

\paragraph{Noisy and Missing Data:}
Based on RSC and RSS property, we can easily extend our theoretical results to the sparse linear regression problem with noisy and missing value in covariates \cite{loh2011high, jain2014iterative}.

==> Outline.tex <==

\subsection{Proof outline}
Here, we give a proof outline for sparse linear regression (\Cref{thm:main_linear}),
and the technique for \Cref{thm:main_logistic} is similar.
The detailed proofs are given in \Cref{sec:proof_stat}.


Since $\param^{t-1}$ and $\parambar^t$ are enforced to be $k'$-sparse, and $\obj$ (the empirical risk defined on $\OGood$) satisfies $\left(\sconvexity,k'\right)$-RSC and $\left(\ssmoothness,k'\right)$-RSM. 
      %we
Combining the two inequalities, we obtain
\begin{align*}
  \obj\left(\parambar^t\right) - \obj\left(\param^*\right)
 \leq \langle \OGrad\left(\param^{t-1}\right), \parambar^t - \param^*\rangle -\frac{\sconvexity}{2}\norm{\param^*-\param^{t-1}}^2_2 +
 \underbrace{ \frac{\ssmoothness}{2}\norm{\parambar^t-\param^{t-1}}^2_2}_{(\diamondsuit)}.
\end{align*}
Expanding the term $(\diamondsuit)$, we have
\begin{align*}
(\diamondsuit)&= \frac{\ssmoothness}{2}
\norm{\param^{t-1} - \param^*}^2_2 -  \frac{\ssmoothness}{2}  \norm{\parambar^t - \param^{t-1}}^2_2 \\
& -\left\langle \RobustG\left(\param^{t-1}\right),\parambar^t-\param^* \right \rangle +\ssmoothness \left\langle \left(\param^{t-1} - \eta \RobustG\left(\param^{t-1}\right)\right) - \parambar^t, \param^*- \parambar^t\right\rangle
\end{align*}
Recall that $\parambar^t$ is directly obtained from hard thresholding, and because $k' = 4\condnum^2 k$, by applying Lemma 1 of \cite{barber2018between} in the last term (more details in \Cref{sec:proof_stat}), we have 
\begin{align*}
   \left\langle \left(\param^{t-1} - \eta \RobustG\left(\param^{t-1}\right)\right) - \parambar^t, \param^*- \parambar^t\right\rangle
    \leq \frac{1}{4\condnum} \norm{\parambar^t - \param^*}^2_2.
\end{align*}
Putting together the pieces, and using
$\Delta^t = \param^t - \param^*$, $\Deltabar^t = \parambar^t - \param^*$,
we obtain the \emph{key inequality}
\begin{align*}
   \obj\left(\parambar^t\right) - \obj\left(\param^*\right) &\leq  \frac{\ssmoothness}{2}\left(\frac{\condnum-1}{\condnum}\norm{\Delta^{t-1}}^2_2 -
\frac{2\condnum-1}{2\condnum}\norm{\Deltabar^t}^2_2 \right) +\underbrace{ \left| \langle {\OGrad}\left(\param^{t-1}\right) - \RobustG\left(\param^{t-1}\right) ,   \Deltabar^t \rangle \right| }_{(\clubsuit)} .
\end{align*}
Next, we use the crucial fact that the perturbation due to outliers (the inner product term $(\clubsuit)$)   is nearly independent of the ambient dimension $d$, because hard thresholding enforces $ \Deltabar^t $ to be $k + k'$ sparse,  resulting in the bound \cref{equ:perturbation}. And this implies
\begin{align}
\label{equ:perturbation_full}
(\clubsuit) \leq \sqrt{k'+k}  \norm{{\OGrad}\left(\param^{t-1}\right) - \RobustG\left(\param^{t-1}\right)}_\infty  \norm{\Deltabar^t}_2. 
\end{align}
Applying \Cref{prop:linear}, and using convexity to obtain a lower bound on $\obj\left(\parambar^t\right) - \obj\left(\param^*\right)$, we can solve a quadratic inequality to obtain the following recursion 
\begin{align*}
     \norm{\Deltabar^t}_2
     \leq
     \left( 1 - \frac{1}{8\rho} \right)\norm{\Delta^{t-1}}_2 +  \frac{4 \Gamma\sigma}{\ssmoothness},      
\end{align*}
which holds with high probability.
Here $\Gamma = O\Big( \sqrt{k'+k}
  \Big( \eps \log (nd) + \sqrt{\frac{\log d}{n}} \Big) \Big)$.
Since Euclidean projection guarantees 
$\norm{\Delta^t}_2 \leq \norm{\Deltabar^t}_2$ \cite{bubeck2015convex}, we have established the global linear convergence rate for \Cref{alg:THT}. Plugging in $\Gamma$, we can obtain the following statistical guarantee 
\begin{align*}
\norm{\widehat{{\param}} - \param^*}_2
= O\left( { \condnum^2 \sigma }
\left( \eps \sqrt{k} \log (nd)  +
\sqrt{\frac{k \log d}{n}}\right)\right).
\end{align*}


